Limiting the Neighborhood: De-Small-World Network for Outbreak Prevention

In this work, we study a basic and practically important strategy to help prevent and/or delay an outbreak in the context of network: limiting the contact between individuals. In this paper, we introduce the average neighborhood size as a new measure for the degree of being small-world and utilize it to formally define the desmall- world network problem. We also prove the NP-hardness of the general reachable pair cut problem and propose a greedy edge betweenness based approach as the benchmark in selecting the candidate edges for solving our problem. Furthermore, we transform the de-small-world network problem as an OR-AND Boolean function maximization problem, which is also an NP-hardness problem. In addition, we develop a numerical relaxation approach to solve the Boolean function maximization and the de-small-world problem. Also, we introduce the short-betweenness, which measures the edge importance in terms of all short paths with distance no greater than a certain threshold, and utilize it to speed up our numerical relaxation approach. The experimental evaluation demonstrates the effectiveness and efficiency of our approaches.

==> related.tex <==
\section{Related Work}
In this section, we review three categories of related work: studies
on disease sreapding and social contagion, inforamtion spreading and local graph extraction.

\noindent{\bf Disease Spreading and Social Contagion}
Infectious disease diffusion has been studied for several decades.
Initially people are interested in modeling the disease spreading process using statistical methods.
\cite{2000} provides a detailed survey on several different models for the spread of infectious disease in populations.
Among these models, SIR (Susceptible/Infective/Removed) proposed in \cite{Anderson1991}, is the simplest model, in which people has three states: 
susceptable, infected and removed, and one state can transfer to another state with contant probability.
Later a more broad process, social contagion is studied, that is the way social networks affect health behavioral 
phenomena, such as smoking cessation, obesity, suicide.
\cite{Smith_Christakis_2008} provides a survey about the effect of social network on human health.
Recently \cite{10.1371/journal.pcbi.1000968} proposes SISa model which is based on disease spreading model as a framework to quantify and predict
the public health affects of socially contagious phenomena.
However, all above works assume that populations are "fully mixed", that is, an infective individual can spread the disease to any other members
in the population, or in a subgroup with equal probability. That means the underlying social network structures are neglected. 
To solve this problem, based on precious works on scale-free networks or small-world networks \cite{PhysRevLett.86.3200, citeulike:5880645},
\cite{citeulike:3053277} varies for individual node the number of connections and infection probability, and exactly solves this problem on SIR
model with percolation theory.

However, different from both diseases spreading and information diffusion, in this paper we take a preventative angle. Instead of studying
the process of disease/information diffusion, we tend to stop the spreading process as soon as possible. 

\noindent{\bf Information Spreading}

Besides disvmease spreaing, information spreading also closely related to our problem, which plays a critical role in human society, 
such as innovation spread, knowledge and information security management, viral marketing, and more \cite{citeulike:126680}. 
\cite{citeulike:8836314} develops an linear influence model by solving a least square regression problem and their method does not utilize 
the underlying network structures. 
By combining the email communication data and personal attribute data, \cite{Wang:2011:ISC} studies the way that the social 
network topological properties (macroscopic level) and individual behavioral profiles (microscopic level) effect information spreading. 
Based tow basic diffusion models, {\it Linear Threshold Mode} and {\it Independent Cascade Model}, \cite{Domingos:2001:MNV,Richardson:2002:MKS,Kempe:2003:MSI} tries to target the people who 
can influence the large fraction of the network to adopt a new product. 

One question we ask about information spreading is: how can we detect misinformation or rumor as soon as possible and stop them? To solve
this similar problem, \cite{Leskovec:2007:COD} tends to detect the most influential nodes in the social network within certain budget.
From \cite{Leskovec:2007:COD} our problem has two obvious differences. 1) Instead of detecting influential vertices, the critical 
edges through which most information passes are detected and removed; therefore, the vertices in our problem are of equal importance. 
2) To prevent the disease/misinformation, we remove the most critical edges at the very beginning. Therefore, we do not need utilizing any diffusion models.

\noindent{\bf Local Graph Extraction}

In this paper, we consider vertex pairs that can be connected with short paths with length at most a small number $l$,
and all these short paths consist of so called "local graph" for this pair.  In spirit, \cite{Andersen_Chung_Lu_2005} solves a very closed problem
to ours. In their problem, assuming that graphs are generated from hybrid model, that is, combined with a random power law graph and a local 
high connectivity graph), authors employ the maximum short flow to extract local graphs. However, in our paper, 1) we do not assume the hybrid model
and 2) we propose a novel method to extract edges that produce high connectivity.

